WANLI: Worker and AI Collaboration for Natural Language Inference Dataset Creation

A recurring challenge of crowdsourcing NLP datasets at scale is that human writers often rely on repetitive patterns when crafting examples, leading to a lack of linguistic diversity. We introduce a novel approach for dataset creation based on worker and AI collaboration, which brings together the generative strength of language models and the evaluative strength of humans. Starting with an existing dataset, MultiNLI for natural language inference (NLI), our approach uses dataset cartography to automatically identify examples that demonstrate challenging reasoning patterns, and instructs GPT-3 to compose new examples with similar patterns. Machine generated examples are then automatically filtered, and finally revised and labeled by human crowdworkers. The resulting dataset, WANLI, consists of 107,885 NLI examples and presents unique empirical strengths over existing NLI datasets. Remarkably, training a model on WANLI improves performance on eight out-of-domain test sets we consider, including by 11% on HANS and 9% on Adversarial NLI, compared to training on the 4x larger MultiNLI. Moreover, it continues to be more effective than MultiNLI augmented with other NLI datasets. Our results demonstrate the promise of leveraging natural language generation techniques and re-imagining the role of humans in the dataset creation process.

==> floats/results_old.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{clcqstuvwxyz}
        \toprule
        &&&\multicolumn{9}{c}{\textbf{Test Set}}\\\cmidrule{4-12}
        &&& \multicolumn{1}{c}{\textbf{Diagnostics}} & \multicolumn{1}{c}{\textbf{HANS}*} & \multicolumn{1}{c}{\textbf{QNLI}*} & \multicolumn{1}{c}{\textbf{WNLI}*} & \multicolumn{1}{c}{\textbf{NQ-NLI}*} & \multicolumn{1}{c}{\textbf{ANLI}} & \multicolumn{1}{c}{\textbf{FEVER-NLI}} & \multicolumn{1}{c}{\textbf{BIG-Bench}*} & \multicolumn{1}{c}{\textbf{\wanli}} \\
        && \multicolumn{1}{r}{Data size $\rightarrow$} & 1104 & 30K & 5266 & 706 & 4855 & 3200 & 20K & 3324 & 5000 \\\midrule
        \multirow{12}{*}{\rotatebox[origin=c]{90}{\textbf{Training Set}}} & MNLI & 393K & 68.47 & 78.08 & 52.69 & 56.09 & 62.34 & 32.37 & 68.29 & 64.68 & 64.62\\
        & \wanli & 103K & \textbf{72.55} & \textbf{89.40} & \textbf{76.81} & \textbf{65.15} & \textbf{64.03} & \textbf{41.12} & \textbf{70.63} & \textbf{75.40} & \cellcolor[gray]{0.8}{75.49}\\\cmidrule{2-12}
        &  MNLI + Tailor & 485K & 67.75 & 79.03 & 54.89 & 56.23 & 63.83 & 32.87 & 68.75 & 72.38 & 64.27 \\
        & MNLI + Z-Aug & 754K & 66.39 & 80.52 & 57.72 & 55.52 & 62.30 & 33.37 & 68.73 & 66.12 & 64.78 \\
        &  MNLI $\diamond$ ANLI & 393K & 67.75 & 79.90 & 68.74 & 60.48 & 62.49 & \cellcolor[gray]{0.8}{54.59} & \cellcolor[gray]{0.8}{72.30} & 72.32 & \textbf{65.96} \\
        &  MNLI + ANLI & 556K & 66.84 & 77.94 & 62.41 & 57.08 & 62.84 & \cellcolor[gray]{0.8}{53.84} & \cellcolor[gray]{0.8}{72.30} & 71.11 & 65.93 \\
        & MNLI $\diamond$ FEVER-NLI & 393K & 66.75 & 76.50 & 56.70 & 57.08 & 61.81 & 35.65 & \cellcolor[gray]{0.8}{76.83} & 58.39 & 63.31 \\
        & MNLI + FEVER-NLI & 601K & 67.57 & 76.05 & 52.90 & 54.95 & 63.02 & 35.37 & \cellcolor[gray]{0.8}{76.93} & 64.65 & 64.53 \\
        & MNLI + SNLI + ANLI & 943K & 68.75 & 78.65 & 63.38 & 58.49 & 62.94 & \cellcolor[gray]{0.8}{54.21} & \cellcolor[gray]{0.8}{72.02} & 71.05 & \textbf{65.10} \\
        & MNLI $\diamond$ \wanli & 393K & 70.19 & 82.25 & \textbf{72.38} & \textbf{61.33} & 63.70 & 36.46 & 71.07 & \textbf{76.17} & \cellcolor[gray]{0.8}{75.49} \\
        & MNLI + \wanli & 496K & \textbf{71.73} & \textbf{82.98} & 64.69 & 60.76 & \textbf{63.91} & \textbf{36.78} & \textbf{71.22} & 70.81 & \cellcolor[gray]{0.8}{75.45}\\\cmidrule{2-12}
        & ANLI & 163K & 65.67 & 80.58 & 81.25 & 66.00 & 62.03 & 55.21 & 72.74 & 77.10 & 63.85\\
        & ANLI + \wanli & 266K & \textbf{72.10} & \textbf{88.50} & \textbf{81.88} & \textbf{67.28} & \textbf{63.39} & \textbf{56.59} & \textbf{73.54} & \textbf{84.89} & \textbf{76.48} \\
        \bottomrule
    \end{tabular}}
    \caption{
    Empirical comparison of different training sets for RoBERTa-large. 
    \textbf{Top}: Comparison of MultiNLI and \wanli as standalone training sets.
    \textbf{Middle}: Comparison of combination schemes with MultiNLI. 
    We consider two data combination strategies, 1) augmentation (+), and 2) random replacement ($\diamond$), where the resulting dataset size is unchanged.
    In the top two sections, we compare generalization to out-of-domain (OOD) challenge sets; gray cells mark settings that do not represent an OOD challenge.
    \textbf{Bottom}: Comparison of whether including \wanli in the training data improves performance on in-domain test data.
    Within each section, the highest accuracy on each test set (excluding gray cells) is bolded.
    Test sets with * contain two label classes: entailment and non-entailment.}
    \label{tab:results}
\end{table*}

==> floats/row4.tex <==
\begin{table*}[]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l}
    \toprule
    \makecell[l]{
    Write a pair of sentences that have the same relationship as the previous examples. Examples:\\[4pt]
    1. In real hearings, adversaries brandish impressive-sounding studies and tell sob stories, rather than \\making buffoonish personal attacks.\\
    Possibility: \textit{\textbf{It should be illegal}} to make buffoonish personal attacks in real hearings. \\[4pt]
    2. You stood by the mantel-piece, twiddling the things on it in your usual fashion, and your hand \\
    shook like a leaf! \\
    Possibility: Your hand shook because you were afraid that \textit{\textbf{you had been caught}}.\\[4pt]
    3. The way he helped me to get on the track of Tuppence and Annette almost disarmed me, but not quite.\\
    Possibility: The way that he helped me to get on the track of Tuppence and Annette \textit{\textbf{was illegal}}.\\[4pt]
    4. Yet it's also noteworthy that the bulk of the recommendations put forth by GAO came from FEMA\\
    regional officials themselves.\\
    Possibility: \textit{\textbf{It was illegal}} for the FEMA officials to get involved with GAO.\\[4pt]
    5. Democrats released documents indicating that Republicans sold big political donors meals\\ 
    with the party's leaders in federal buildings in 1995.\\
    Possibility: \textit{\textbf{It is illegal}} for a party to solicit products to donors.\\[4pt]
    6.}\\
    \bottomrule
    \end{tabular}}
    \caption{Context corresponding to row 4 in \autoref{tab:examples}, which contains \colorbox{neu}{\textit{Neutral}} examples where the hypothesis states or implies that something mentioned in the premise is illegal or wrong.}
    \label{tab:row4}
\end{table*}

==> floats/row6.tex <==
\begin{table*}[]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l}
    \toprule
    \makecell[l]{
    Write a pair of sentences that have the same relationship as the previous examples. Examples:\\[4pt]
    1. Those employees will have to be cross-trained so that they can \textbf{\textit{handle both their return processing}} \\
    \textbf{\textit{and compliance responsibilities}}.\\
    Possibility: Those employees will have to be trained so that they can \textbf{\textit{make burgers}}.\\[4pt]
    2. This would narrow the wedge between the individual's return on saving and \textbf{\textit{society's return on}} \\
    \textit{\textbf{investment that results from the taxation of income from saving}}.\\
    Possibility: This would narrow the wedge between the individual's return on saving and \textit{\textbf{how many pairs of}} \\
    \textbf{\textit{shoes people own}}\\[4pt]
    3. LSC representation of aliens is limited to certain classes of aliens who broadly may be described \\
    as lawful permanent residents, prospective lawful permanent residents and one specific group \\
    of temporary, nonimmigrants.\\
    Possibility: The LSC represents aliens who are lawful residents, and also enjoy chai tea. \\[4pt]
    4. In addition to establishing a more complete reporting system, LSC is committed to using economic \\
    analysis and performance measures to \textit{\textbf{evaluate the impact of federal funding and individual grantee}}\\
    \textit{\textbf{performance}}.\\
    Possibility: LSC is committed to using economic analysis for the use of \textit{\textbf{how many burgers one can eat.}}\\[4pt]
    5. 8 The balanced scorecard is a tool to measure performance at various levels of an organization and to \\
    \textit{\textbf{provide employees with data to help them achieve individual and organizational results.}}\\
    Possibility: The balanced scorecard is a tool to measure performance of an organisation and \textit{\textbf{how fast}} \\
    \textit{\textbf{you can tap dance}}\\[4pt]
    6.}\\
    \bottomrule
    \end{tabular}}
    \caption{Context corresponding to row 4 in \autoref{tab:examples}, in which the hypothesis offers a different purpose for something than in the premise.}
    \label{tab:row6}
\end{table*}

==> sections/old/2.method.tex <==
\section{Worker-AI Collaborative Dataset Creation}
\label{sec:method}
\swabha{since we went with only one dataset, worth thinking about merging this section with section 3...}

Our goal is to create examples which would enhance model robustness on unseen distributions.
We outline a four-stage pipeline for dataset creation, which requires as prerequisites an initial dataset $\mathcal D_0$ and a strong task model $\mathcal M$ trained on $\mathcal D_0$. 
First, we automatically \textbf{collect} groups of examples exemplifying challenging reasoning patterns in $\mathcal D_0$ relative to $\mathcal M$, using data maps (\citealp{swayamdipta-etal-2020-dataset}; Stage 1, see \S\ref{subsec:seed_collection}).
Then we \textbf{overgenerate} similar examples by leveraging the pattern replication capabilities of GPT-3 \cite{brown-etal-2020-language} (Stage 2; \S\ref{subsec:overgeneration}). 
While GPT-3 can generate examples efficiently, it may not reliably replicate the desired pattern and its output quality will not be uniform.
We address this by automatically \textbf{filtering} the generated examples using a metric derived from data maps (Stage 3; \S\ref{subsec:filtering}).
We finally subject the collected data to \textbf{human review}, in which crowdworkers optionally revise examples and assign gold labels (Stage 4; \S\ref{sec:human_review}).

\paragraph{Dataset Cartography.} 
\citet{swayamdipta-etal-2020-dataset} introduced data maps which automatically analyze different regions in a dataset, w.r.t.\ the behavior of a classification model during training. 
Based on two metrics---the mean and variance of the confidence of the model in the correct label, across training epochs---data maps reveal different regions in a dataset.
These include \textit{easy-to-learn} examples which the model consistently predicts correctly through training, \textit{hard-to-learn} examples on which it is consistently incorrect, and \textit{ambiguous} examples for which the model's confidence in the correct answer exhibits high \textit{variability} across train epochs.
A key component of our pipeline relies on ambiguous examples, which were shown to lead to more robust models. 
Additionally, ambiguous examples contain fewer spurious correlations \cite{gardner-etal-2021-competency}, suggesting that they capture under-represented counterexamples to spurious correlations.
Indeed, such counterexamples take more epochs of training to learn and are crucial for generalization \cite{tu-etal-2020-empirical}, providing a potential explanation for why they appear ambiguous across early epochs and lead to more robust models. 
\swabha{below is also removed, why? :(}
% Finally, ambiguous examples have desirable properties from an information-theoretic perspective \cite{ethayarajh2021informationtheoretic}. 

\subsection{Stage 1: Collection of Exemplars}
\label{subsec:seed_collection}


In this stage, we automatically collect groups of examples from $\mathcal D_0$ which represent linguistic patterns we wish to include in the target dataset.
We begin with a seed example $(x_i,y_i)\in\mathcal D_0$ belonging to the most ambiguous $p\%$ relative to $\mathcal M$.
% To generate a new example with the same reasoning pattern, we wish to leverage the ability of GPT-3 \cite{brown-etal-2020-language} for in-context learning; hence, we need to first collect examples that test a similar kind of reasoning to $x_i$.\swabha{already addressed above}
In order to collect examples that test a similar kind of reasoning to $x_i$, we use the \texttt{[CLS]} token representation of each example relative to the \textit{task} model $\mathcal M$, and find the $k$-nearest neighbors via cosine similarity to $x_i$ that \textit{have the same label}.
% \swabha{too specific; consider keeping it a little general: internal model representation from $\mathcal M$.}\alisa{other model representations are untested; it might be crucial that the representation we use is exactly the input to the prediction head, i.e. the final encoding of the example relative to the task. also we only qualitatively inspect this one representation.}
Detailed qualitative inspection shows that the nearest neighbors in this representation space tend to capture a human-interpretable similarity in the \textit{reasoning} required to solve an example, rather than lexical or semantic similarity (examples in \autoref{tab:examples}).
\citet{han-tsvetkov-2021-influence-tuning} give another interpretation for this approach: for examples with the same label, the similarity of \texttt{[CLS]} token embeddings actually represents the similarity of \textit{gradient updates} in the row of the final projection layer corresponding to that label.
Thus, two examples are close if training on them would ``update'' the final layer of the model similarly.

By automatically identifying areas for augmentation, our method does not require any prior knowledge of challenging patterns and makes our method tractable for building on top of large-scale datasets.
Nonetheless, exemplar collection could potentially be approached in different ways (e.g., through expert curation or category labels).


\subsection{Stage 2: Overgeneration}
\label{subsec:overgeneration}

% \swabha{should we even specify GPT-3 here? any powerful language model that allows few-shot prompting should work here, right?}\alisa{I think that's obvious, so specifying GPT-3 is okay? it makes writing way easier}
% \nascomment{worth pointing out that we just need a conentional (left-to-right) language model (nothing is GPT-3 specific) is good, see my revision below}

Given an automatically extracted group of $k+1$ examples from the original dataset $\mathcal D_0$, we construct a natural language context (prompt) for a left-to-right language model; in this work, we use GPT-3.
Our method leverages GPT-3 in way that is distinct from its typical usage in few-shot settings, where given examples demonstrating a task, GPT-3 performs the task on a new, unlabeled example.
Here, we instead give GPT-3 examples representing a particular subcategory of the task, and ask GPT-3 to \textit{generate} a new example within the same subcategory. 
% \swabha{slice or sub-category of the task? sub-task?}
% While the prompt consists of examples that share a label, the label is not necessarily shown to the language model.
% \alisa{sorry noah -- actually, the template is slightly different for each label (see figure 2). this was because it was really hard to get gpt-3 to generate contradictions otherwise.}
% \nascomment{make clearer up front that it's just the text \emph{inputs} that are going in to GPT-3, and we're mainly using it to generate \emph{more inputs}. you get to the outputs in a minute, but it will be clearer if you say inputs repeatedly here}
For each context, we sample from GPT-3 to create $n$ distinct examples.\swabha{somewhere in the appendix specify the decoding settings under GPT-3, as well as dates of access of the API, for reproducibility.}\alisa{done, check Appendix \ref{subsec:generation_hyperparams}}
Although generated examples at this stage could be assumed to share label of its $k+1$ in-context examples, we instead consider the resulting dataset $\mathcal{D}\textsubscript{gen}=\{x_i\}_i$ at the end of Stage 1 to be \emph{unlabeled}.
% We will acquire human annotated gold-standard labels (Stage 4; \S\ref{subsec:annotation}).


\subsection{Stage 3: Automatic Filtering}
\label{subsec:filtering}
% \swabha{"map-based filtering" sounds confusing, either specify "data map" or just say "filtering", because otherwise map means nothing?}
In this step, we wish to filter generated examples from Stage 2 to retain those that are the most ambiguous with respect to $\mathcal M$. 
However, computing ambiguity for an example requires that it be a part of the original training set, whereas we wish to estimate the ambiguity of an \textit{unlabeled} example \textit{without} additional training.
Thus we introduce a new metric called \textbf{estimated max variability}, which measures the worst-case spread of predictions on an example $x_i$ across checkpoints of a trained model. 
Let $E$ be the total epochs in training, $\mathcal Y$ the label set, and $p_{\theta^{(e)}}$ the probability assigned with parameters $\theta^{(e)}$ at the end of the $e$-th epoch. 
We define the estimated max variability as:
\begin{equation}
    \sigma_i=\max_{y\in \mathcal Y}\sigma\left(\left\{p_{\theta^{(e)}}(y\mid x_i)\right\}_{e\in E}\right),
\end{equation}
\noindent where $\sigma$ is the standard deviation function. 

Concretely, we \textit{retroactively} compute the prediction from each saved epoch of $\mathcal M$ on $x_i$.  
The only assumption made is that the single example, if it had been a part of the training set, would have made a negligible difference on each model checkpoint (at least as observed through its posterior probabilities).\footnote{Indeed, we find a high correlation between variability and estimated max variability; see \autoref{sec:max_variability}.}
In taking a maximum across labels, we consider $x_i$ to be ambiguous as long as $\mathcal M$ is undecided on \textit{any} label $\in \mathcal{Y}$.


Our resulting dataset, $\mathcal D\textsubscript{filtered}\subseteq\mathcal D\textsubscript{gen}$
retains an equal number of examples from each (intended) label class with the highest estimated max variability, such that $\mathcal D\textsubscript{filtered}$ is a fraction $q$ of the size of $\mathcal D\textsubscript{gen}$.
\swabha{wait, does this mean we are balancing out the dataset wrt the intended label? And Table 2 stats are showing that humans think otherwise?}\alisa{yep! see \S\ref{subsec:imbalance}}

\subsection{Stage 4: Human Review}
\label{sec:human_review}

As the final stage of our pipeline, we recruit human annotators to review each unlabeled example $x_i\in\mathcal D\textsubscript{filtered}$, and assign it a label $y_i$. %, with the aim of producing gold-standard labels, as well as ensuring data quality.\alisa{I feel like we've already said this a lot, maybe? and we say it again in the next sentence}
The annotator may optionally revise $x_i$ to create a higher-quality example $x_i'$, or let $x_i' = x_i$. 
\swabha{defined how? either define here or point to appendix where instructions are specified?}\alisa{the instructions are in the appendix, and linked in section 3}
% They may also discard examples that are extremely low quality (based on fluency, completeness, etc.) and would require substantial revision.\alisa{I feel like saying this in WaNLI is enough?}
This results in our final dataset $\mathcal D\textsubscript{collab}=\{(x_i',y_i)\}_i$.
In general, we believe the degree \swabha{changed from "role of revision" to "degree"} of revision depends on the quality of machine-generated examples. 
Indeed, we need to strike a balance between leveraging human capabilities and avoiding the re-emergence of annotation artifacts that may come with too much freedom in revision.


==> sections/old/3.wanli.tex <==
\section{\wanli}
\label{sec:wanli}

We implement our pipeline (\S\ref{sec:method}) to create \wanli, new dataset for natural language inference (NLI).
The task involves predicting whether a premise \textit{entails}, \textit{contradicts} or is \textit{neutral} to a hypothesis.
% Despite great progress on the task, NLI models still struggle on out-of-domain instances, suggesting they have overfit to existing datasets \cite{gururangan-etal-2018-annotation, poliak-etal-2018-hypothesis}.
NLI has broad applicability in NLP: it has proven useful for pretraining \cite{clark-etal-2019-boolq,phang-etal-2018-sentence}, and can be applied to verify answers in question-answering \cite{chen-etal-2021-nli-models} and factuality of generated summaries \cite{maynez-etal-2020-faithfulness}.
% We introduce \wanli, \textbf{W}orker-and-\textbf{A}I \textbf{NLI}, a new and more challenging dataset for natural language inference, based on our four-stage pipeline.

As our initial dataset $\mathcal D_0$, we use MultiNLI \cite{williams-etal-2018-broad}, a large-scale multi-genre dataset for the NLI task.
We finetune RoBERTa-large \cite{liu-etal-2019-roberta} on MultiNLI for our task model $\mathcal M$ (training details in \autoref{sec:modeling_details}).


\subsection{Stage 1: Collection of Exemplars}
\label{subsec:wanli_seed_collection}

As seed examples, we use MultiNLI examples in the top $p=25\%$ for ambiguity w.r.t\ RoBERTa-large.\footnote{For exemplar collection, we exclude the telephone genre of MultiNLI, which consists of telephone conversation transcripts, due to their low fluency and ill-defined entailment relationships.
During pilots, we found that generated examples mimicking telephone conversations would require crowdworkers to revise low-quality text for basic fluency.}
For each seed example, we collect the $k=4$ nearest same-label neighbors based on the \texttt{[CLS]} embedding from $\mathcal M$, for a total of 5 in-context examples for GPT-3. 
We apply the prompt template shown in \autoref{fig:template}, and order the examples in \textit{increasing} similarity to the seed example.
% \swabha{missing: how many total in-context prompts do you use?}\alisa{``This is approximately 10K seed examples, each corresponding to a GPT-3 context.'' I could say this, but I thought it was inferrable from the writing.}


\subsection{Stage 2: Overgeneration}
\label{subsec:wanli_overgeneration}

We use GPT-3 Curie (the second-largest GPT-3 model) and use top-$p$ decoding \cite{holtzman-etal-2020-curious} with $p=0.5$
(additional details in Appendix \ref{subsec:generation_hyperparams}).
For each set of in-context examples, we sample $n=5$ new examples to create $\mathcal D\textsubscript{gen}$.

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/template.png}
    \caption{
    Prompt template instructing GPT-3 to generate a new example, given a set of in-context examples. 
    To separate the premise and hypothesis, the word ``Implication'' is used for entailment examples (shown here), ``Possibility'' for neutral examples, and ``Contradiction'' for contradiction examples.}
    \label{fig:template}
\end{figure}

\subsection{Stage 3: Automatic Filtering}
\label{subsec:wanli_filtering}
% \swabha{this has a different name from what we call it in the previous section.}\alisa{it's because the filtering at this stage isn't just map-based, we also do heuristic-based filtering. but I changed it anyway.}

We first employ simple heuristics to discard examples exhibiting observable failure cases of GPT-3.
Specifically, we discard examples where 1) the premise and hypothesis are identical, sans punctuation or casing, 2) the generated example is an exact copy of an in-context example, 3) the example contains some phrases from the instruction (e.g., ``pair of sentences''), and 4) the premise or hypothesis is shorter than 5 characters. 
Then, we compute the estimated max variability (\S\ref{subsec:filtering}) for the remaining examples with respect to $M$, and retain generations with values in the top half ($q=0.5$).

% \swabha{"map-based filtering" sounds confusing, either specify "data map" or just say "filtering", because otherwise map means nothing?}
In this step, we wish to filter generated examples from Stage 2 to retain those that are the most ambiguous with respect to $\mathcal M$. 
However, computing ambiguity for an example requires that it be a part of the original training set, whereas we wish to estimate the ambiguity of an \textit{unlabeled} example \textit{without} additional training.
Thus we introduce a new metric called \textbf{estimated max variability}, which measures the worst-case spread of predictions on an example $x_i$ across checkpoints of a trained model. 
Let $E$ be the total epochs in training, $\mathcal Y$ the label set, and $p_{\theta^{(e)}}$ the probability assigned with parameters $\theta^{e}$ at the end of the $e$-th epoch. 
We define the estimated max variability as:
\begin{equation}
    \sigma_i=\max_{y\in \mathcal Y}\sigma\left(\left\{p_{\theta^{(e)}}(y\mid x_i)\right\}_{e\in E}\right),
\end{equation}
\noindent where $\sigma$ is the standard deviation function. 

Concretely, we \textit{retroactively} compute the prediction from each saved epoch of $\mathcal M$ on $x_i$.  
The only assumption made is that the single example, if it had been a part of the training set, would have made a negligible difference on each model checkpoint (at least as observed through its posterior probabilities).\footnote{Indeed, we find a high correlation between variability and estimated max variability; see \autoref{sec:max_variability}.}
In taking a maximum across labels, we consider $x_i$ to be ambiguous as long as $\mathcal M$ is undecided on \textit{any} label $\in \mathcal{Y}$.


Our resulting dataset, $\mathcal D\textsubscript{filtered}\subseteq\mathcal D\textsubscript{gen}$
retains an equal number of examples from each (intended) label class with the highest estimated max variability, such that $\mathcal D\textsubscript{filtered}$ is a fraction $q$ of the size of $\mathcal D\textsubscript{gen}$.
\swabha{wait, does this mean we are balancing out the dataset wrt the intended label? And Table 2 stats are showing that humans think otherwise?}\alisa{yep! see \S\ref{subsec:imbalance}}

\subsection{Stage 4: Human Review}
\label{subsec:wanli_validation}
We use the Amazon Mechanical Turk platform for human annotation (details about crowdworkers and guidelines in \autoref{sec:human_annotation}).
Given an unlabeled example, annotators are asked to optionally revise it for quality, while preserving the intended meaning as much as possible through minimal revisions.\footnote{In pilots, we found that when annotators exercised too much freedom in revision, they often re-introduced the same artifacts that have been well-documented in NLI.}
Then, annotators assign a label.
Alternatively, if an example would require a great deal of revision to fix \textit{or} if it could be perceived as offensive, they were asked to discard it.

Two distinct annotators label each example in $\mathcal D\textsubscript{filtered}$. 
For examples that both annotators labeled without revision, we achieved a Cohen Kappa score of $0.60$, indicating substantial agreement.

To create the final dataset $\mathcal D\textsubscript{collab}$, we discard an example if \textit{either} annotator chose to discard it, and we keep a revision only if \textit{both} annotators revise an example (and choose a revision uniformly at random).
When both annotators label the example as-is but choose different labels, we sample one of the two labels uniformly at random. 
\swabha{is this still the case? I thought we would include both labels in the dataset, but to train the model we would randomly use one... what we do for training need not be exactly the same as what is in the dataset}
The rationale for this is discussed in Appendix \ref{subsec:disagreement_more}.

\input{floats/dataset_statistics}

Crowdworkers annotate a total of 118,724 examples. 
Of these, 108,079 (91.03\%) are labeled and presented in $\mathcal D\textsubscript{collab}$ and the remaining 8.97\% are discarded. 
Of the labeled examples, 3.65\% were revised. 
We randomly split the data into a train and test sets. 
% \swabha{so we don't create a counterfactuals test set?}\alisa{not for now, discussed over slack}
Key dataset statistics are summarized in \autoref{tab:dataset_statistics}.
Unlike MultiNLI and SNLI, \wanli is not label-balanced; see \autoref{subsec:imbalance} for a discussion.
% \swabha{something specifically about how our resulting dataset is not label balanced, unlike MultiNLI and SNLI. This could be similar to how NLI instances might be distributed realistically...}\alisa{I don't have a lot of confidence about describing a ``natural distribution'' for NLI instances.}\swabha{fair, can we still highlight the imbalance of label classes? I think it's an important point that we need to preemptively declare before some reviewer points it out}\alisa{done, check?}

\input{floats/results}

==> sections/old/5.discussion.tex <==
\section{What does \wanli show about the human machine collaboration pipeline?}
\label{sec:discussion}

We discuss observations from collecting \wanli that may shed insight for future work in the direction of collaborative dataset creation.

\subsection{What kinds of revisions do annotators tend to make?}
\label{subsec:what-revisions?}

We find that revisions fall broadly into two categories: improving the fluency of the text, and improving the clarity of the entailment relationship. 
The majority of revisions change the length only slightly, with $74\%$ of both premise revisions and hypothesis revisions changing the word count between $-1$ and $+2$ words. 
Fluency revisions often target well-documented issues with text generation, such as redundancy and self-contradiction.
Clarity revisions often resolve ambiguities in the example that make the entailment relationship difficult (or impossible) to determine, such as ambiguous coreference or temporal references.
We provide examples of revisions in Appendix \ref{subsec:revision_more}.

\subsection{What kinds of examples do annotators disagree on?}
\label{subsec:disagreement}

We find that examples on which annotators disagree provide an extremely interesting test bed for analyzing inherent disagreements in NLI (see Appendix \ref{subsec:disagreement_more}).
Upon inspecting the examples on which annotators disagreed, we observe that many examples represent genuinely ambiguous cases rather than careless mislabels, echoing previous findings \cite{pavlick-kwiatkowski-2019-inherent}.
Future work could further investigate these disagreements, and learning strategies that take into account the inherent ambiguity of these examples.

% \subsection{How does performance vary with \wanli dataset size?}
% We train RoBERTa-large on differently-sized subsets of \wanli. \nascomment{lifting this note to a comment to make sure it's addressed: [Not really sure what comments to make here...] ... my answer is that this is only interesting if you show similar curves for MNLI on its own ... also I think these should ideally have error bars.  I think the main interesting finding would be that low-$n$ \wanli is better than low-$n$ MNLI.  you could speculate about what would happen if you doubled the data again, but I'm not sure that's wise.}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{figures/dataset_size.png}
%     \caption{Performance of RoBERTa-large trained on \wanli, for different training set sizes. Note that for binary datasets, accuracy starts at $50\%$; for three-label datasets, accuracy starts at $33\%$.}
%     \label{fig:dataset_size}
% \end{figure}

\subsection{How reliably does GPT-3 reproduce the in-context pattern?}
\label{subsec:in-context}

One characteristic of \wanli is its imbalanced label distribution: even though the set of seed examples for generation was constructed to be balanced, after undergoing human labeling, only 15.35\% of examples are given the contradiction label.
We observe that contradiction patterns in in-context examples are generally much more challenging for GPT-3 to copy, likely because it was trained on (mostly) coherent sequences of sentences.
More broadly, we find that more abstract reasoning patterns are harder for GPT-3 to mimic than patterns that involve simpler transformations.

Nonetheless, even when GPT-3 does not successfully copy the examples, the diverse set of in-context examples leads to a variety of creative output that may be challenging for human crowdworkers to achieve.
